Perceptual Quality Assessment of HEVC and VVC Standards for 8K Video

With the growing data consumption of emerging video applications and users requirement for higher resolutions, up to 8K, a huge effort has been made in video compression technologies. Recently, versatile video coding (VVC) has been standardized by the moving picture expert group (MPEG), providing a significant improvement in compression performance over its predecessor high efficiency video coding (HEVC). In this paper, we provide a comparative subjective quality evaluation between VVC and HEVC standards for 8K resolution videos. In addition, we evaluate the perceived quality improvement offered by 8K over UHD 4K resolution. The compression performance of both VVC and HEVC standards has been conducted in random access (RA) coding configuration, using their respective reference software, VVC test model (VTM-11) and HEVC test model (HM-16.20). Objective measurements, using PSNR, MS-SSIM and VMAF metrics have shown that the bitrate gains offered by VVC over HEVC for 8K video content are around 31%, 26% and 35%, respectively. Subjectively, VVC offers an average of 40% of bitrate reduction over HEVC for the same visual quality. A compression gain of 50% has been reached for some tested video sequences regarding a Student t-test analysis. In addition, for most tested scenes, a significant visual difference between uncompressed 4K and 8K has been noticed.

==> tables/LayeredKimono_wassim.tex <==
\begin{tabular}[t]{lrrrrrr}
\diagbox[width=\dimexpr \textwidth/8+2\tabcolsep\relax, height=0.6cm]{HEVC}{VVC} &  R1 &  R2 &  R3 &  R4 &    4K &   REF \\
\midrule
R1 &    \bfseries\cellcolor{redtable}{0.00} &    \bfseries\cellcolor{redtable}{0.00} &    \bfseries\cellcolor{redtable}{0.00} &    \bfseries\cellcolor{redtable}{0.00} &   \bfseries\cellcolor{redtable}{0.00} &   \bfseries\cellcolor{redtable}{0.00} \\
R2 &    \bfseries\cellcolor{redtable}{0.01} &    \bfseries\cellcolor{redtable}{0.00} &    \bfseries\cellcolor{redtable}{0.00} &    \bfseries\cellcolor{redtable}{0.00} &   \bfseries\cellcolor{redtable}{0.00} &   \bfseries\cellcolor{redtable}{0.00} \\
R3 &    \bfseries\cellcolor{redtable}{0.01} &    \bfseries\cellcolor{greentable}{0.34} &    \bfseries\cellcolor{redtable}{0.01} &    \bfseries\cellcolor{redtable}{0.01} &   \bfseries\cellcolor{redtable}{0.01} &   \bfseries\cellcolor{redtable}{0.00} \\
R4 &    \bfseries\cellcolor{redtable}{0.00} &    \bfseries\cellcolor{redtable}{0.00} &    \bfseries\cellcolor{greentable}{0.81} &    \bfseries\cellcolor{greentable}{0.99} &   \bfseries\cellcolor{greentable}{0.80} &   \bfseries\cellcolor{redtable}{0.01} \\
4K     &    \bfseries\cellcolor{redtable}{0.00} &    \bfseries\cellcolor{redtable}{0.00} &    \bfseries\cellcolor{greentable}{0.98} &    \bfseries\cellcolor{greentable}{0.86} &   \bfseries\cellcolor{greentable}{1.00} &   \bfseries\cellcolor{redtable}{0.03} \\
REF    &    \bfseries\cellcolor{redtable}{0.00} &    \bfseries\cellcolor{redtable}{0.00} &    \bfseries\cellcolor{greentable}{0.05} &    \bfseries\cellcolor{greentable}{0.11} &   \bfseries\cellcolor{redtable}{0.03} &   \bfseries\cellcolor{greentable}{1.00} \\
\hline
\end{tabular}

